Cross-section measurements of the Higgs boson decaying into a pair of tau-leptons in proton-proton collisions at $\sqrt{s}=13$ TeV with the ATLAS detector

A measurement of production cross sections of the Higgs boson in proton-proton collisions is presented in the $H\rightarrow\tau\tau$ decay channel. The analysis is performed using $36.1\mathrm{fb}^{-1}$ of data recorded by the ATLAS experiment at the Large Hadron Collider at a center-of-mass energy of $\sqrt{s}=13$ TeV. All combinations of leptonic ($\tau \rightarrow l \nu \bar{\nu}$ with $l = e$, $\mu$) and hadronic ($\tau \to \mathrm{hadrons} \nu$) tau decays are considered. The $H\rightarrow\tau\tau$ signal over the expected background from other Standard Model processes is established with an observed (expected) significance of 4.4 (4.1) standard deviations. Combined with results obtained using data taken at 7 and 8 TeV center-of-mass energies, the observed (expected) significance amounts to 6.4 (5.4) standard deviations and constitutes an observation of $H\rightarrow\tau\tau$ decays. Using the data taken at $\sqrt{s}=13$ TeV, the total cross section in the $H\rightarrow\tau\tau$ decay channel is measured to be $3.77^{+0.60}_{-0.59}\mathrm{(stat.)}^{+0.87}_{-0.74}\mathrm{(syst.)}\mathrm{pb}$, for a Higgs boson of mass 125 GeV assuming the relative contributions of its production modes as predicted by the Standard Model. Total cross sections in the $H\rightarrow\tau\tau$ decay channel are determined separately for vector-boson-fusion production and gluon-gluon-fusion production to be $0.28 \pm 0.09\mathrm{(stat.)}^{+0.11}_{-0.09}\mathrm{(syst.)}\mathrm{pb}$ and $3.1 \pm 1.0\mathrm{(stat.)}^{+1.6}_{-1.3}\mathrm{(syst.)}\mathrm{pb}$, respectively. Similarly, results of a fit are reported in the framework of simplified template cross sections. All measurements are in agreement with Standard Model expectations.

==> acknowledgements/Makefile <==
# Makefile for creating ATLAS Acknowledegments

TEXLIVE  = 2013
LATEX    = latex
PDFLATEX = pdflatex
BIBTEX   = biber
DVIPS    = dvips
DVIPDF   = dvipdf

BASENAME = Acknowledgements-main

.PHONY: clean cleanpdf

run_pdflatex: $(BASENAME).pdf
	@echo "Made $<"

# Change TeX Live version
texlive: $(BASENAME).tex
	if [ $(TEXLIVE) -ge 2007 -a $(TEXLIVE) -lt 2100 ]; then \
	  echo "Changing texlive value in $$file"; \
	  sed -i'.bak' 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' $<; \
	else echo "Invalid value for TEXLIVE: $(TEXLIVE)"; fi; \

# Standard LaTeX targets
$(BASENAME).pdf: $(BASENAME).tex
	$(PDFLATEX) $<
	-$(BIBTEX)  $(basename $<)
	$(PDFLATEX) $<
	$(PDFLATEX) $<

%.bbl: %.tex *.bib
	$(PDFLATEX) $*
	$(BIBTEX) $*

clean:
	-rm *.dvi *.toc *.aux *.log *.out *.blg *.bbl *.bcf *-blx.bib \
	 *.run.xml *.synctex.gz *~

cleanpdf:
	-rm $(BASENAME).pdf

cleanall: clean cleanpdf

